Multi S-Graphs: An Efficient Distributed Semantic-Relational Collaborative SLAM

Collaborative Simultaneous Localization and Mapping (CSLAM) is critical to enable multiple robots to operate in complex environments. Most CSLAM techniques rely on raw sensor measurement or low-level features such as keyframe descriptors, which can lead to wrong loop closures due to the lack of deep understanding of the environment. Moreover, the exchange of these measurements and low-level features among the robots requires the transmission of a significant amount of data, which limits the scalability of the system. To overcome these limitations, we present Multi S-Graphs, a decentralized CSLAM system that utilizes high-level semantic-relational information embedded in the four-layered hierarchical and optimizable situational graphs for cooperative map generation and localization in structured environments while minimizing the information exchanged between the robots. To support this, we present a novel room-based descriptor which, along with its connected walls, is used to perform inter-robot loop closures, addressing the challenges of multi-robot kidnapped problem initialization. Multiple experiments in simulated and real environments validate the improvement in accuracy and robustness of the proposed approach while reducing the amount of data exchanged between robots compared to other state-of-the-art approaches. Software available within a docker image: https://github.com/snt-arg/multi_s_graphs_docker

==> notas.tex <==
Rosbags para experimentos

Hriday:
- Real: C1F1 [stugalux_oetrage_f1_4r]
        C1F2 [stugalux_oetrage_f2_3r] (el clásico)
        C2F1 [stugalux_urchat_f1_2r] (no tiene paredes) 
        C2F2 [stugalux_urchat_f2_2r] (Es el principal del paper de Sgraph)
        C3F1, 
        C3F2
- Simulation: C1F0 [stugalux_oetrage_f1_4r]
              C1F2, 
              SE1, 
              SE2, 
              SE3, 
              + Paul's
